The Wrappingness and Trunkenness of Volume-Preserving Flows

Link invariants of long pieces of orbits of a volume-preserving flow can be used to define diffeomorphism invariants of the flow. In this paper, we extend the notions of wrapping number and trunk and define invariants of links with respect to a fibration on a 3-manifold. Extending work of Dehornoy and Rechtman, we apply this to define diffeomorphism invariants wrappingness and trunkenness of volume-preserving flows on 3-manifolds and interpret these invariants as obstructions to the existence of a global surface of section for the flow. Finally, we construct flows and show that wrappingness and trunkenness are not functions of the helicity of a flow.

==> overflow.tex <==
\begin{comment}
\begin{remark}
    The space $S^1$ is a $K(\ZZ,1)$ and homotopy classes of maps $[Y:S^1]$ are in 1-1 correspondence with elements of $H^1(Y,\ZZ)$.  If two fibrations $\pi,\pi': Y \rightarrow S^1$ represent the same cohomology class $[\pi] = [\pi'] \in H^1(Y,S^1)$, then the fiber surfaces $\pi^{-1}(\theta)$ and $\pi'^{-1}(\theta)$ are homologous, incompressable surfaces in a 3-manifold, hence they are isotopic.  One can then use the 3-dimensional Smale conjecture, proved by Hatcher \cite{Hatcher}, to prove that the fibrations $\pi,\pi'$ are in fact isotopic.
\end{remark}

\end{comment}

\begin{comment}
\begin{lemma}
The linking number is given by
\[ [\beta] \cdot \mu = \lim_{\epsilon \rightarrow 0} \frac{1}{\epsilon}\int_{\Phi_x^{[0,\epsilon]}(P_{\theta})} \beta(X) d \mu\]
where $\beta$ is Poincare dual to $P_{\theta}$
\end{lemma}


\begin{lemma}
We have the following inequalities
\[ [\pi] \cdot \mu \leq Wrp(X,\mu,\pi) \leq Tks(X,\mu,\pi)\]
\end{lemma}

\begin{proof}
In order to compute the linking number, it suffices to let $\beta$ be Poincare dual to some fiber.  We can then see that the flux through any given fiber is bounded below by the linking integral.  The second inequality follows immediately from the definition.

Consider the set
\[\underset{n \rightarrow + \infty}{\lim} \, \frac{1}{T_n} \, \underset{\epsilon \rightarrow 0}{\lim} \, \frac{1}{\epsilon} \mu \left( K(T_n,p) \cap \phi^{[0,\epsilon]}(\pi^{-1}(\theta) )\right)\]

\end{proof}
\end{comment}


\begin{comment} We can further show that trunkenness with respect to a fibered link is not a function of the linking number and helicity of the flows.

 \begin{theorem}
    Let $L \subset Y$ be a fibered link supporting a tight contact structure $(Y,\xi)$.  There exists a Reeb flow $R_{\alpha}$ and volume-preserving flow $\widetilde{R}$ such that
    \begin{enumerate}
        \item $L$ is a union of periodic orbits of $R_{\alpha}$ and $\widetilde{R}$,
        \item $R_{\alpha}$ and $\widetilde{R}$ are homotopic through nonvanishing vector fields in the complement of $L$,
        \item the linking numbers of $R_{\alpha}$ and $\widetilde{R}$ with respect to $L$ and the helicities of $R_{\alpha}$ and $\widetilde{R}$ agree.
    \end{enumerate}
but the trunkenness of $R_{\alpha}$ and $\widetilde{R}$ with respect to the open book decomposition $(L,\pi)$ do not agree.
\end{theorem}

\end{comment}

\begin{comment}
\subsection{Further directions}

Given a flow $\phi$ on $Y$, there exist homotopy obstructions to isotoping a fibration $\pi$ until all the pages are transverse to the flow.  In Section \ref{sec:homotopy}, we give a concrete interpretion the Thom-Pontryagin construction to describe the homotopy obstruction.  However, there should be further geometric obstructions to the flow admitting a surface of section.

We can describe one heuristically as follows.  Let $F$ be the set of points along with the flow is tangent to the fibration.  Generically, this is a surface in $Y$.  We can decompose $F$ into two subsets, the {\it entry set} $F^{in}$ and the {\it exit set} $F^{out}$, according to whether the flow is positively and negatively transverse to $F$.  The boundary between these is the set of points where the flow is tangent to $F$ (and the fibration). Let $Y_+$ and $Y_-$ be the subsets where the flow is positive and negative transverse, respectively, to the fibration.  Then there is some obstruction determined by the inclusion
\[H_1(F^{out}) \rightarrow H_1(Y_+)\]
Specifically, given a simple closed curve $\gamma$ in $F^{out}$, the flow $\phi^{[0,t]}(\gamma)$ is an annulus and $\phi^t(\gamma)$ is a curve in $Y^+$ for small $t$.  However, if $[\phi^t(\gamma)]$ is algebraically linked with $Y_-$, then the flow must take some point in $\gamma$ back into $Y_-$.

\end{comment}



\begin{comment}
\subsection{Topological decompositions}

A 3-manifold $Y$ is a {\it graph manifold} if it can be decomposed into the union $Y = Y_1 \cup \dots \cup Y_n$ of Seifert-fibered spaces glued along torus boundary components.  Morgan shows that a 3-manifold $Y$ is a graph manifold if and only if it admits a so-called round handle decomposition \cite{Morgan}.  The potential round handle decompositions of $S^3$ were classified independently by Wada \cite{Wada} and Yano \cite{Yano}.  Moreover, Wada described the class of links in $S^3$ that arise as the core circles of a round handle decomposition.  By examining the proof, we can identify the class of links that arise as the cores of round handle decompositions that can be built from the basic building blocks $A$ and $B$ (and $C$).

For a given link $L$, we will consider partitions of $L$ into {\it even} and {\it odd} components.  An even component corresponds to the core circle of some building block $A \cong S^1 \times D^2$.  An odd component corresponds to a generic fiber of building block $B \cong S^1 \times P$.  

\begin{theorem}[Wada]
    Let $H$ denote the Hopf link with both components even.  Let $\cB$ denote the set of partitioned links in $S^3$ generated by $H_{0,2}$ and the following two operations:
    \begin{enumerate}
       \item if $L_1,L_2 \in \cB$ and $K_1 \subset L_1$ and $K_2 \subset L_2$ are components, both even, then
        \[(L_1 \# L_2) \cup m \in \cB\]
        where the connect sum is performed along $K_1$ and $K_2$ and $m$ is an odd meridian of $K_1 \# K_2$,
        \item if $L \in \cB$ and $K \subset L$ be an even component.  Then $L_{K,p,q} \in \cB$, where $L_{K,p,q}$ is the union of $L$ with two $(p,q)$-cables of $K$, one odd and the other even.
    \end{enumerate}
If $L \subset \cB$, there exists a round handle decomposition of $S^3$ corresponding to a fat round handle decomposition into the building blocks $A$ and $B$, such that $L$ is the core indexed link of the round handle decomposition.
\end{theorem}

\begin{proof}
This result is implied in the proof of the main theorem of \cite{Wada}.  In particular, the two operations in the above theorem are Wada's operations IV and V, which correspond to the fat round 1-handle $S^1 \times P$. 
\end{proof}

Recall that a link $L \subset S^3$ is {\it algebraic} if there exists a polynomial $f: \CC^2 \rightarrow \CC$ with an isolated singularity at the origin and $L$ is the link of this singularity.  It is known that algebraic links are precisely the iterated positive cables of the unknot and moreover that each is fibered.  

\begin{proposition}
    Let $L$ be an algebraic link and $H$ be the Hopf link.  There exists a link $\widetilde{L} \subset \cB$ containing the split union $L \cup H$ as an even sublink
\end{proposition}

\begin{proof}
    Applying the first operation to two copies of the Hopf link $H$, we obtain a link $L_1 \in \cB$ that contains two disjoint, even unknots $U_1$ and $U_2$. By repeatedly applying the second operation to $U_1$, we can obtain any iterated torus knot.  Applying the first operation and connect summing a Hopf link to $U_2$, we obtain a Hopf link as a sublink that is split from the iterated torus knot. 
\end{proof}

\end{comment}


\begin{comment}

The contribution of the building block $B$ to the global helicity of $d \alpha$ is then
\[Hel(d \alpha) = \int_B (\alpha + \beta) \wedge d \alpha \]
where $\beta$ is a closed 1-form.  We can choose a basis for $H^1_{DR}(B)$ that restrict to the 1-forms $d \theta, d \psi_1, d \psi_2$ on $\partial B$.  Therefore, by abuse of notation we set
\[\beta = M d \theta + N_1 d \psi_1 + N_2 d \psi_2\]
Therefore
\begin{align*}
    \int_B \alpha \wedge d\alpha &= 2 \pi \int_P (\phi - \phi'h) \\
    \int_B \beta \wedge d \alpha &= - \int_{\partial B} (M d \theta + N_1 d \psi_1 + N_2 d \psi_2) \wedge \alpha \\
    &= 4\pi^2 \left( N_1 \phi_1(0) + N_2 \psi_2(0) + M (h_1(0) + h_2(0) + h_3(0))\right)
\end{align*}

\end{comment}

\begin{comment}
\begin{example}
    Take $f(t) = a(1 - qt)$ and $g(t) = b(1 - qt)$ so
    \[F = at - \frac{aq}{2} t^2 \qquad G = bt - \frac{bq}{2} t^2\]
    Then
    \[\int_0^1 Gf - fG dt = \int_0^1 (abt - abqt - \frac{abq}{2}t^2 + \frac{abq^2}\]
\end{example}

\begin{example}
\label{ex:helicity-turn}
    Take $f(t) = \cos(at + b)$ and $g(t) = \sin(at + b)$ so
    \[F(t) = \frac{1}{a} \sin(at + b) \qquad G(t) = -\frac{1}{a} \cos(at + b)\]
    Then
\[
        \int_0^1(Gf - fg) dt = \int_0^1 -\frac{1}{a}\left( \cos^2(at + b) + \sin^2(at + b)\right)dt = -\frac{1}{a}
\]
\end{example}

\end{comment}
